Bayesian Disturbance Injection: Robust Imitation Learning of Flexible Policies

Scenarios requiring humans to choose from multiple seemingly optimal actions are commonplace, however standard imitation learning often fails to capture this behavior. Instead, an over-reliance on replicating expert actions induces inflexible and unstable policies, leading to poor generalizability in an application. To address the problem, this paper presents the first imitation learning framework that incorporates Bayesian variational inference for learning flexible non-parametric multi-action policies, while simultaneously robustifying the policies against sources of error, by introducing and optimizing disturbances to create a richer demonstration dataset. This combinatorial approach forces the policy to adapt to challenging situations, enabling stable multi-action policies to be learned efficiently. The effectiveness of our proposed method is evaluated through simulations and real-robot experiments for a table-sweep task using the UR3 6-DOF robotic arm. Results show that, through improved flexibility and robustness, the learning performance and control safety are better than comparison methods.

==> sections/Formulation_v1.tex <==
%--------------------------------------------------------------------------------------------------
% \subsection{Behavior Cloning with Gaussian Process Regression}
% In this section, we provide a brief overview of Behavior Cloning (BC) with Gaussian Processes Regression (GPR).

% \subsection{Bayesian learning frameworks}
% In a Bayesian learning framework, a policy is defined as a probability distribution of action outputs, and a probabilistic generative model of the data is constructed to probabilistically infer the posterior distribution of the policy from the supervised data based on Bayesian theory.

% \subsection{Behavior Cloning (BC)}
\subsection{Problem statement}
Behavior cloning (BC) is one of the imitation learning methods in which a robot learns a control policy that imitates the human's actions by using empirical data of the human's demonstration, and it has been applied to the field of robotics \cite{bain1995framework}.
The objective of BC is to learn policies to imitate the action from the expert's demonstration data.
A policy decides an action $a_t$ on state $\mathbf s_t$, and $\pi_{\theta}({a}_t \mid \mathbf{s}_{t})$ and $\pi_{\theta^*}({a}_t \mid \mathbf{s}_{t})$ are the learning policy and the expert's policy respectively.
The state transitions with initial state probability $p(\mathbf{s}_0)$ and state transition probability $p(\mathbf{s}_{t+1}\mid\mathbf{s}_{t}, {a}_t)$ with Markov property.
Let trajectory $\tau=(\mathbf{s}_{0},{a}_{0},\mathbf{s}_{1},{a}_{1}\dots {a}_{T-1},\mathbf{s}_{T})$ be the time sequence of the state and action data when the robot executes $T$ steps from the initial state $\mathbf{s}_0$ from the policy $\pi_{\theta}({a}_t \mid \mathbf{s}_{t})$, and define the probability of the trajectory as follows.
\begin{equation}\label{BC:loss}
    p(\tau\mid\pi_{\theta})=p\left(\mathbf{s}_{0}\right) \prod_{t=0}^{T-1} \pi_{\theta} \left({a}_t \mid \mathbf{s}_{t}\right) p\left(\mathbf{s}_{t+1} \mid {a}_t, \mathbf{s}_{t}\right)
\end{equation}

To calculate the difference between the action $a^{*}_t\sim \pi_{\theta^*}(a_t\mid\mathbf{s}_t)$ taken from the expert and the action $a^{\theta}_t\sim \pi_{\theta}(a_t\mid\mathbf{s}_t)$ taken from the learned policy, L2 norm $l(a^*_t, a^{\theta}_t)=||a^*_t - a^{\theta}_t||^2_2$ is applied.
Let $J(\theta) = -\sum_{t=0}^{T-1} l(a^*_t, a^{\theta}_t)$ be the evaluation function of the parameter $\theta$.
Then, we can obtain the optimal policy parameter $\hat\theta$ with demonstration data by the expert, as follows:
\begin{equation}\label{BC:objective_function}
    \hat{\theta}
    = \argmax_\theta\mathbb{E}_{p(\tau\mid\pi_{\theta^{*}})}
    \left[J(\theta )\right]
\end{equation}

The discrepancy between the probability $p(\tau\mid\pi_{\theta^{*}})$ of the trajectory for training in BC and the probability $p(\tau\mid\pi_{\hat{\theta}})$ of the trajectory for testing the policy is called the covariate shift \cite{ross2010efficient}.
A robot's learned policy with large covariate shifts in BC due to perturbation, model approximation error, or differences in initial conditions may be placed in a never experienced state, in which there is a risk that it may take action to damage itself or an environment.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{BC with injection noise}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Addressing the problem caused by the covariate shift, the method injects noise into the expert's action to expand the robot's state during the expert's demonstration. It optimizes the injection noise parameters using an iterative method. Finally, Policies trained with the above dataset are robust to state shifts induced by perturbation and model approximation errors during testing \cite{laskey2017dart}.
% Let $\pi_{\theta^*}(a_n\mid\mathbf{s}_n,\sigma^2)=\mathcal{N}(a^*_n,\sigma^2)$ indicate Gaussian noise-injected expert's policy.
% Let $p(\tau\mid\pi_{\theta^*},\sigma_k^2)$ be the probability distribution of trajectories with $\pi_{\theta^*}$

% \begin{align}\label{DART:Policy_objective_function}
%     {\theta}^{R}
%     = \argmax_\theta\mathbb{E}_{ p(\tau\mid\pi_{\theta^{*}},{\sigma}^2)}
%     \left[J(\theta )\right]
% \end{align}
\begin{align}
&\mathrm{Covariate~shift}\nonumber\\
&=\left|E_{p\left(\tau \mid \pi_{\theta^{*}}, \sigma ^2\right)} \left[J(\theta )\right]-E_{p\left(\tau \mid \pi_{\theta^{R}}\right)} \left[J(\theta )\right]\right|
\end{align}
First, an initial noise with appropriate initial parameters is injected into the expert's action, and $N$ demonstrations are collected.
Note that this paper utilizes Gaussian noise, which is injected into the expert's action.
Next, policy $\pi_{\theta}$ is learned by minimizing the loss (\ref{BC:loss}).
The learned policy is used to optimize the noise parameter.
Once the noise parameter is optimized, N demonstrations are collected from the noise-injected expert, and the robot is trained on the aggregate training dataset.
This algorithm is repeated K times.


Let the training dataset as $\mathcal{D}=[\mathbf{a^*},\mathbf{S}]$, where $\mathbf{a^*}=[a^*_n]_{n=1}^{N_k}$ and $\mathbf{S}=[\mathbf{s}_n]_{n=1}^{N_k}$ represent all actions and states of a expert performing a task for $k$ times.

Optimize the noise parameter (the variance of the noise distribution) for each expert's demonstration, and let $\pi_{\theta^*}(a_n\mid\mathbf{s}_n,\sigma_k^2)=\mathcal{N}(a^*_n,\sigma_k^2)$ indicate the expert's policy employed for the $k$~th trial.

Let $p(\tau\mid\pi_{\theta^*},\sigma_k^2)$ be the probability distribution of trajectories with $\pi_{\theta^*}$, and $p(\mathcal{D}\mid\pi_{\theta^{*}},\{{\sigma}_{k}^2\})$ be the probability distribution of trajectories collected over $k$~th trials.
Here, $\{{\sigma}_{k}^2\}=\{{\sigma}_{1}^2,{\sigma}_{2}^2,\cdots,{\sigma}_{k}^2\}$ is the noise parameter used for $k$~th trials.

DART find the parameters of the optimal policy, $\hat{\theta_k}$, using the same evaluation function as standard BC.
\begin{align}\label{DART:Policy_objective_function}
    \hat{\theta}_k
    = \argmax_\theta\mathbb{E}_{ p(\mathcal{D}\mid\pi_{\theta^{*}},\{{\sigma}_{k}^2\})}
    \left[J(\theta )
    \right]
\end{align}

The log-likelihood of the noise parameter $\sigma^2$ is defined as $\log \mathcal{N}(a^{k}_n\mid a^*_n, \sigma^2)$, using a conditional probability distribution in which the learned actions $a^{k}_n$ from (\ref{DART:Policy_objective_function}) are input as variables in the distribution of the noise-injected expert's policy.

The noise parameter is optimized with a maximum expectation of this log-likelihood on the probability distribution of $k$~trajectories collected on the $k$~th trial as: 
\begin{equation}\label{DART:Noise_objective_function}
    \hat{\sigma}_{k+1}^2
    = \argmax_\sigma\mathbb{E}_{ p(\tau\mid\pi_{\theta^{*}},\sigma_{k}^2)}
    \left[\sum_{n=N_{k-1}}^{N_k}\log \mathcal{N}(a^{k}_n\mid a^*_n, \sigma^2)
    \right]
\end{equation}

Using the fact that the value of the log-likelihood does not change even if the mean and the input of the log-likelihood are replaced, the log-likelihood for the parameter $\theta_k,\{{\sigma}_{k+1}^2\}$ is derived as :

\begin{align}\label{GP-DART:likelihood}
    \log p(\mathbf{a}^*\mid\mathbf{S},{\theta_k},\{{\sigma}_{k+1}^2\}) &=\sum^{k}_{j=1} \sum^{N_j}_{n=N_{j-1}}\log \mathcal{N}(a^*_n\mid a^{k}_n,\sigma_{j+1}^2)\nonumber\\
    &=\log \mathcal{N}(\mathbf{a}^*\mid\mathbf{a}^{k},\Psi)
\end{align}
where, $\{{\sigma}_{k+1}^2\}, \Psi$ are respectively :

\begin{equation}\label{MGP:variance_set}
    \{\sigma_{k+1}^2\}=\{\sigma_2^2,\sigma_3^2, \cdots, \sigma_{k+1}^2\}
\end{equation}
\begin{equation}
    \Psi = 
        \begin{bmatrix}
        \sigma_2^2 \mathbf{I}_{T}  & 0 & \cdots & 0\\
         0& \sigma_3^2 \mathbf{I}_{T} & \cdots & 0\\
        \vdots  & \vdots & \ddots & \vdots \\
        0  & 0 & \cdots & \sigma_{k+1}^2 \mathbf{I}_{T}
        \end{bmatrix}
\end{equation}

Therefore, optimization of parameters $\theta_k,\sigma_{k+1}^2$ derived as :
\begin{equation}\label{GP-DART:objective_function}
    \begin{split}
        &\hat{\theta}_k,\{\hat{\sigma}_{k+1}^2\}\\
        &= \argmax_{\theta_k,\{{\sigma}_{k+1}^2\}}\mathbb{E}_{p(\mathcal{D}\mid\pi_{\theta^{*}},\{{\sigma}_{k}^2\})}
        \left[
        \log p(\mathbf{a}^*\mid\mathbf{S},{\theta_k},\{{\sigma}_{k+1}^2\})
        \right]
    \end{split}
\end{equation}

% Non-Bayesian parametric methods such as the maximum likelihood method (e.g (\ref{DART:Policy_objective_function})) rely on point estimates of the parameter $\hat{\theta}_k$.
% This can lead to models being over-fitted, which requires designing an appropriate policy model for each task and makes it difficult to learn the policy in tasks where there are multiple optimal actions.

% \subsection{Bayesian non-parametric method}
% The Bayesian non-parametric method defines the prior distribution of the parameter, and then estimates the posterior distribution of the parameter directly from the data based on the Bayes' theorem.
% By marginalizing the parameters using the posterior distribution of the parameters, the predictive distribution for the new state $s_{*}$ can be obtained analytically.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{PROPOSED METHOD}
In this section, we propose an algorithm, MGP-DART, which uses infinite overlapping mixtures of Gaussian processes \cite{ross2013nonparametric} as the policy model and employs variational Bayesian learning to simultaneously optimize the policy and noise parameters.

\subsection{Injection Noise Conditional Generative Model}
In order to use infinite overlapping mixtures of Gaussian processes, we denote the set of regression functions with $\{ {\mathbf{F}}^{(m)}\}=\left\{\mathbf{f}^{(m)}(\mathbf{S}) \right\}^{\infty}_{m=1}$ instead of the parametric policy $\pi_{\theta}$, and the prior distribution is given by :
\begin{equation}\label{prior_GP}
    p\left(\left\{\mathbf{F}^{(m)}\right\} \relmiddle|\mathbf{S}\right)=\prod_{m=1}^{\infty}  \mathcal{N}\left(\mathbf{f}^{(m)} \relmiddle|\mathbf{0},\mathbf{K}^{(m)}; \{\boldsymbol{\omega}^{(m)}\}\right)
\end{equation}
where $\mathbf{K}^{(m)}=\mathrm{k}^{(m)}({\mathbf{S}}, {\mathbf{S}})$ is the $m$~th kernel gram matrix and $\mathrm{k}^{(m)}({\mathbf{S}}, {\mathbf{S}})$ is a kernel function with the hyperparameter $\omega^{(m)}$.
Let $\{\boldsymbol{\omega}^{(m)}\}$ be the hyperparameter of an infinite number of kernel functions.

Then we define a binary indicator matrix $\mathbf{Z}$ to represent the association between the data and the regression function, and let (\ref{prior_z}), based on the Stick Breaking Process (SBP), be the prior of $\mathbf{Z}$, which can be interpreted as an infinite mixture model to estimate the number of mixtures of the regression functions.
\begin{equation}\label{prior_z}
    p(\mathbf{Z} \mid \mathbf{v})
    = \prod_{n=1}^{N} \prod_{m=1}^{\infty}\left(v_{m} \prod_{j=1}^{m-1}\left(1-v_{j}\right)\right)^{\mathbf{Z}_{n,m}}    
\end{equation}
\begin{equation}\label{prior_v}
    p(\mathbf{v} \mid \alpha)=\prod_{m=1}^{\infty} \operatorname{Beta}\left(v_{m} \relmiddle| 1,\alpha\right)
\end{equation}

In practice, since we cannot deal with infinite-dimensional vectors in variational Bayesian learning, it is necessary to replace the $\infty$ component with a predetermined upper bound of the mixtures, $M$.
${{v}_m}$ is a random variable indicating the probability that the data corresponds to the $m$~th GP, and $\alpha$ is a hyperparameter of SBP denoting the level of concentration of the data in the set.

Therefore, the likelihood conditional on $\{{\mathbf{F}}^{(m)}\},\mathbf{Z}$ as : 
\begin{equation}\label{MGP-DART:likelihood}
    p\left({\mathbf{a}^*} \relmiddle|\{\mathbf{F}^{(m)}\}, \mathbf{Z}; \{{\sigma}_{k+1}^2\} \right) =
    \prod_{n=1}^{N}\prod_{m=1}^{\infty} \mathcal{N}\left({\mathbf{a}_n^*} \relmiddle| \mathbf{f}_n^{(m)}, \Psi \right)^{\mathbf{Z}_{n, m}}
\end{equation}
We can describe such a formulation in a graphical model that defines the relationship between the variables as shown in Fig.~\ref{fig:concept}, and the joint distribution of the model as :
\begin{align}\label{joint_distribution}
    &p\left({\mathbf{a}^*}, \mathbf{Z}, \mathbf{v},\{\mathbf{F}^{(m)}\}\relmiddle|\mathbf{S} ;\Omega \right) \nonumber\\
    &~~~~~~=p\left({\mathbf{a}^*} \relmiddle|\{\mathbf{F}^{(m)}\}, \mathbf{Z}; \{{\sigma}_{k+1}^2\} \right) \nonumber\\
    &~~~~~~~~~~~~~p\left(\left\{\mathbf{F}^{(m)}\right\} \relmiddle|\mathbf{S}; \{\boldsymbol{\omega}^{(m)}\}\right)
    p(\mathbf{Z} \mid \mathbf{v}) p(\mathbf{v} \mid \alpha)
\end{align}
where $\Omega =(\{\boldsymbol{\omega}^{(m)}\},\{{\sigma}_{k+1}^2\},\alpha)$ represents a set of hyperparameters.
% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=\hsize]{Figure/Generative_model.pdf}
%     \caption{Graphical model of MGP-DART}
%     \label{fig:generative_model}
% \end{figure}
\begin{figure*}[tb]
    \centering
    \includegraphics[width=\hsize]{Figure/Concept_Figure.pdf}
    \caption{Overview of MGP-DART}
    \label{fig:concept}
\end{figure*}
Bayesian learning is a framework that estimates the posterior distributions of the policies and their predictive distributions for the input of new data, rather than seeking the parameters of the policies as in (\ref{GP-DART:objective_function}).
In order to obtain the posterior and predictive distributions, it is necessary to calculate the log marginal likelihood as :
\begin{align}\label{marginal_likelihood}
    p({\mathbf{a}^*}\mid\mathbf{S};\Omega )= \iiint p\left({\mathbf{a}^*}, \mathbf{Z}, \mathbf{v},\{\mathbf{F}^{(m)}\}\relmiddle|\mathbf{S} ;\Omega \right)
    d \mathbf{Z} d \mathbf{v} d\{\mathbf{F}^{(m)}\}
\end{align}
In addition, the following (\ref{marginal_likelihood}) is also used to optimize the hyperparameter $\Omega$.
\begin{align}
    \hat{\Omega}
    &= \argmax_{\Omega}\mathbb{E}_{p(\mathcal{D}\mid\pi_{\theta^{*}},\{{\sigma}_{k}^2\})}
    \left[
    \log {
    p({\mathbf{a}^*}\mid\mathbf{S};\Omega )
    }
    \right]
\end{align}
However, it is intractable to calculate the log marginal likelihood of (\ref{marginal_likelihood}) analytically.
In the next section, we derive a variational lower bound for variational Bayesian learning and use it to iteratively perform hyperparameter optimization by approximating the true posterior distribution of latent variables, such as the expectation-maximization (EM) algorithm.

==> sections/Formulation_v2.tex <==
% \begin{itemize}
%     \item 学習した政策を誤りの発生源に対してロバスト化するために、人間がdemonstrationする行動にノイズを注入し、専門家がこの摂動からどのように回復するかを学習する、persistence excitation[7]という現象はRobotics 分野で利用されている。
%     \item 適当にノイズを入れれば良いわけではなく、ノイズをどんな方向にどんな大きさで加えるのか最適化する必要がある。
% \end{itemize}

\subsection{Imitation Learning from An Expert's Demonstration}
The objective of imitation learning is to learn an control policy by imitating the action from the expert's demonstration data.
A dynamics model is denoted as Markovian with a state $\mathbf s_t \in \mathbb{R}^{Q}$, an action $a_t \in \mathbb{R}$ and a state transition distribution $p(\mathbf s_{t+1}\mid \mathbf s_t, a_t)$.
A policy $\pi(a_t\mid\mathbf s_t)$ decides an action from a state.
A trajectory $\tau=(\mathbf{s}_{0},{a}_{0},\mathbf{s}_{1},{a}_{1}\dots {a}_{T-1},\mathbf{s}_{T})$ which is a sequence of state action pairs of $T$ steps.
The trajectory distribution is indicated as:
\begin{align}
    p(\tau\mid\pi)=p(\mathbf{s}_0)\prod_{t=0}^{T-1}\pi(a_t\mid\mathbf{s}_t)p(\mathbf{s}_{t+1}\mid\mathbf{s}_t,a_t).
\end{align}

Imitation learning is the method which learns a policy using an expert's demonstration data.
% We denote the policy evaluation function which indicates similarity with a policy and collected trajectory as:
We define the function which computes the similarity of two policies using given trajectory as:
\begin{align}
    J(\pi,\pi^{\prime},\tau) = -\sum_{t=0}^{T-1} \mathbb E_{\pi(a\mid \mathbf s_t),\pi^{\prime}(a'\mid \mathbf s_t)}\left[||a - a'||_{2}^{2}\right].
\end{align}
A learned policy $\pi^R$ is obtained by solving following optimization problem using a trajectory collected by an expert's policy $\pi^*$:
\begin{align}\label{BC:policy}
    \pi^{R}= \argmax_\pi\mathbb{E}_{p(\tau\mid\pi^*)}\left[J(\pi,\pi^{*},\tau)\right].
\end{align}

In imitation learning a learned policy has problem of error compound caused by covariate shift which is the difference of the trajectory distribution in data collection and testing as:
\begin{equation}
    \left|\mathbb{E}_{ p(\tau\mid\pi^*)}[J(\pi^{R},\pi^{*},\tau)] -\mathbb{E}_{ p(\tau\mid\pi^R)}[J(\pi^{R},\pi^{*},\tau)]\right|.
\end{equation}


% \subsection{Problem Statement}
% A policy $\pi : \mathcal{S} \longrightarrow \mathcal{A}$ decides an action $a_t \in \mathcal{A}$ on corresponding to a state $\mathbf{s}_t\in \mathcal{S}$.
% The state transitions with initial state probability $p(\mathbf{s}_0)$ and state transition probability $p(\mathbf{s}_{t+1}\mid\mathbf{s}_{t}, {a}_t)$ with Markov property.
% Let trajectory $\tau=(\mathbf{s}_{0},{a}_{0},\mathbf{s}_{1},{a}_{1},\dots,{a}_{T-1},\mathbf{s}_{T})$ be the time sequence of the state and action data when the robot executes $T$ steps from the initial state $\mathbf{s}_0$ from the policy $\pi$, and define the probability of the trajectory as :
% \begin{equation}
%     % p(\tau;\pi)=p(\mathbf{s}_0)\prod_{t=0}^{T-1}p_{\pi}(a_t|\mathbf{s}_t)p(\mathbf{s}_{t+1}|\mathbf{s}_t,a_t)   
%     p(\tau\mid\pi)=p(\mathbf{s}_0)\prod_{t=0}^{T-1}\pi(a_t\mid\mathbf{s}_t)p(\mathbf{s}_{t+1}\mid\mathbf{s}_t,a_t)
% \end{equation}
% $\pi(a_t\mid\mathbf{s}_t)$ is a probabilistic distribution that sample action from a given state.

% \subsection{Imitation Learning from Expert's Demonstration}
% Imitation learning aims for the robot to learn skills by observing expert's demonstration \cite{bain1995framework}.
% Expert steers the robot to collect trajectory $\tau^* = \{\mathbf{s}_t,a_t^*\}_{t=0}^{T-1}$ , a series of state $\mathbf{s}_t$ and action $a_t^*$.
% The policy's evaluation function  (i.e., the similarity between the expert and the policy $\pi$ ) is induced by applying the L2 norm as :
% \begin{equation}
%     % J(\pi) = -\sum_{t=0}^{T-1} ||a^*_t - \pi(\mathbf{s}_t)||_{2}^{2}
%     J(\pi,\tau) = -\sum_{t=0}^{T-1} \mathbb E_{\pi(a_t'\mid \mathbf s_t)}[~||a_t - a_t'||_{2}^{2}~]
%     % l(\mathbf{a}_t^*, \pi(\mathbf{s}_t)) = ||a^*_t - \pi(\mathbf{s}_t)||_{2}^{2}
% \end{equation}

% Then, we can obtain the learned-policy $\pi^{R}$ with expert's demonstration data, as follows:
% \begin{align}\label{BC:policy}
%     % \pi^{R}=\underset{\pi}{\argmax} \mathbb{E}_{p\left(\tau ; \pi^{*}\right)}[J(\pi,\pi^*, \tau)]
%     % \pi^{R}=\underset{\pi}{\argmax} \mathbb{E}_{\mathbf{S}\sim p\left(\tau ; \pi^{*}\right)}[J(\pi,\mathbf{S})]
%     \pi^{R}= \argmax_\pi\mathbb{E}_{p(\tau\mid\pi^*)}[J(\pi,\tau)]
% \end{align}

\begin{figure*}[t]
    \centering
    % \includegraphics[width=0.9\hsize]{Figure/Concept_Figure_v2.pdf}
    \includegraphics[width=0.9\hsize]{Figure/Concept_Figure_v3.pdf}
    \caption{Overview of MGP-DART: Training data sets $\mathcal{D}$ collected up to the k iterations of injecting noise into the expert's actions are used to estimate the policy and learn the k noise parameters. The last noise parameter $\sigma_k^2$ is used for the noise to be injected into the next iteration.}
    \label{fig:concept}
\end{figure*}

\subsection{Robust Imitation Learning by Injecting Noise into Expert}
To learn policy robustly to error compound caused by covariate shift, the novel imitation learning method which is called DART is proposed \cite{laskey2017dart}.
The method collects an expert demonstration with injected noise to actions.
The level of injected noise is optimized iteratively to reduce covariate shift during data collection.
% The optimized noise level is derived as the approximation error of learned policy.


% Injecting noise to an expert's demonstrated action and learning how the expert recovers from this perturbation is known to robustify the learned policies against sources of error; the phenomenon of persistence excitation \cite{sastry2011adaptive}.
% DART \cite{laskey2017dart} is the method that learns policy robustly for an error caused by the covariate shift by repeating optimization of the injection noise distribution and the expert's demonstration data collection with noise injection. 
% Specifically, an optimization procedure computes the optimal noise for given trajectories. Then, the demonstration is repeated with this optimized noise added to the expert action, and this iterative process is repeated for K times.
% Specifically, the optimization procedure:
% \begin{inparaenum}
% \item Compute the optimal noise for a given trajectory, and
% \item Add this optimized noise into the expert action at the demonstration.
% \end{inparaenum}
% the objective of the DART is minimize covariate shift
% These two iterative processes are repeated K times.

The method assumes that the injected noise is sampled from Gaussian distribution as $\epsilon_t\sim\mathcal N(0, \sigma^2_k)$ due to learn policy robustly to any  disturbance in the system, where $k$ is the number of optimizations.
The injected noise $\epsilon_t$ is added to the expert's action $a^*_t$.

We denote the noise injeccted expert's trajectory distribution as $p(\tau\mid\pi^*,\sigma^2_k)$ and the trajectory distribution with learned policy as $p(\tau\mid\pi^R_k)$.
To reduce covariate shift, DART introduces upper bound of covariate shift by Pinsker's inequality as:


% The method assumes that the injected noise in the $k$-th data collection is sampled from Gaussian distribution as $\epsilon_t\sim\mathcal N(0, \sigma^2_k)$ and the injection noise $\epsilon_t$ is added to the expert's action.
% The parameter of the inject noise distribution is optimized to reduce covariate shift with the trajectory distribution with the noise injection $p(\tau\mid\pi^*,\sigma^2_k)$ and the trajectory distribution with learned policy $p(\tau\mid\pi^R_k)$.
% By introducing Pinsker's inequality, DART employs upper bound instead of the covariate shift as:
\begin{align}\label{DART:covariate}
    &\left|\mathbb E_{p(\tau\mid\pi^*,\sigma^2_k)} \left[J(\pi^{R},\pi^{*},\tau)\right]-\mathbb E_{p(\tau\mid\pi^R_k)} \left[J(\pi^{R},\pi^{*},\tau)\right]\right|\nonumber\\
    &\leq T \sqrt{\frac{1}{2} \mathrm{KL}\left(p(\tau\mid\pi^R_k) \mid\mid p(\tau\mid\pi^*,\sigma^2_k)\right)},
\end{align}
where, $\mathrm{KL}(\cdot\mid\mid\cdot)$ is Kullback-Leibler divergence.
However, the upper bound is intractable since the learned policy's trajectory distribution $p(\tau\mid\pi^R_k)$ is unknown.
Therefore, DART solves the upper bound using the noise injected expert's trajectory distribution instead of the learned policy's trajectory distribution.
Optimal injection noise distribution is optimized as:
% However, the upper bound is intractable since the expectation of the learned policy's trajectory distribution cannot be solved.
% Hence, DART iteratively evaluates the expectation from the expert's trajectory distribution with the previous noise parameter $\sigma^2_{k-1}$.
% Based on the upper bound, the injection noise distribution is optimized as:
\begin{align}\label{DART:Noise}
    &\sigma_{k}^{2} =\argmax_{\sigma^{2}} \mathbb{E}_{p(\tau\mid\pi^{*},\sigma^2_{k-1})} \nonumber \\
    &~~~~~\left[\sum_{t=0}^{T-1} \mathbb E_{\pi^R_{k}(a_t'\mid\mathbf s_t)} [\log \mathcal{N}\left( a_t'\relmiddle| a_t, \sigma^{2}\right)]\right].
\end{align}
The optimized injected noise distribution can be interpreted as the likelihood of learned policy.

The learned policy $\pi^R_k$ used in the optimization of $\sigma^2_k$ is obtained by following:
\begin{align}\label{DART:policy}
    \pi^R_k= \argmax_\pi\sum_{i=1}^{k-1}\mathbb{E}_{p(\tau\mid\pi^*,\sigma_i^2)}[J(\pi,\pi^{*},\tau)].
\end{align}

% \color{black}

% \subsection{Robust Imitation Learning Injecting Noise into Expert}
% Collecting training dataset by adding noise to Expert will include in the training dataset the action of recovering from an aberrant trajectory than Noise.
% Injecting noise is optimized in an Iterative approach so as to reduce the covariate shift.
% The Covariate shift indicates how much the trained distribution differs from the actual test distribution $p(\tau\mid\pi^R)$ , is defined as :
% \begin{equation}
%     \left|\mathbb{E}_{ p(\tau\mid\pi^*)}[J(\pi^R,\tau)] -\mathbb{E}_{ p(\tau\mid\pi^R)}[J(\pi^*,\tau)]\right|
% \end{equation}
% We define a distribution $p(\tau^* ;  \sigma^2)$ that samples the training data using policy $\pi(a_t\mid a_t^*;\sigma^2) = \mathcal{N}(a_t\mid a_t^*,\sigma^2)$ , which adds Gaussian noise to Expert's action.
% Then the noise parameter $\sigma^2$ conditional covariate shift satisfies :
% \begin{align}\label{DART:covariate}
%     &\left|\mathbb E_{p(\tau\mid\pi^*,\sigma^2)} \left[J(\pi^R,\tau)\right]-\mathbb E_{p\left(\tau\mid\pi^R \right)} \left[J(\pi^*,\tau)\right]\right|\nonumber\\
%     &\leq T \sqrt{\frac{1}{2} \mathcal{D}_{\mathcal{KL}}\left(p(\tau\mid\pi^R), p(\tau\mid\pi^*,\sigma^2)\right)}
% \end{align}
% Reduces covariate shift by seeking the noise parameter $\hat{\sigma}^2$ that minimizes KL-Divergence (\ref{DART:covariate}).
% The noise parameters are gradually optimized by repeating the process $k$~times from collecting data via the noise-injected expert to optimizing the noise.
% Let the training dataset as $\mathcal{D}=[\mathbf{a^*},\mathbf{S}]$, where $\mathbf{a^*}=[a^*_n]_{n=1}^{N_k}$ and $\mathbf{S}=[\mathbf{s}_n]_{n=1}^{N_k}$ represent all actions and states of a expert performing a task for $k$~times.
% Let $p(\mathcal{D})=\prod_{i=1}^{k}p(\tau|\pi^*,\sigma_i^2)$ be the probability distribution of trajectories collected over $k$~th trials.
% Here, $\{{\sigma}_{k}^2\}=\{{\sigma}_{i}^2\}_{i=1}^{k}$ is the set of noise parameters used for $k$~th iteration.
% Learning policy from training dataset $\mathcal{D}$ based on (\ref{BC:policy}) ($\pi^k = \pi^R$).
% \begin{align}\label{DART:policy}
%     \pi^{k}= \argmax_\pi\mathbb{E}_{\tau \sim p(\mathcal{D})}[J(\pi,\tau)]
% \end{align}
% We derive the likelihood of the learned-policy $\pi^k$ from the training data collected by injecting the Gaussian noise with the current noise parameter $\sigma_{k}^2$ as follows:
% \begin{align}\label{DART:Noise}
%     &\sigma_{k+1}^{2}\nonumber\\
%     &=\argmax_{\sigma^{2}} \mathbb{E}_{p(\tau| \pi^{*},\sigma^2_{k})}\left[\sum_{t=0}^{T-1} \mathbb E_{\pi^k(a_t'\mid\mathbf s_t)} [\log \mathcal{N}\left( a_t'\relmiddle| a_t, \sigma^{2}\right)]\right]
% \end{align}


%============================================================================
% Sasaki's workspace
% 先生が読みやすく一旦comment out しました。
%============================================================================
% \color{red}
% \section{Proposed Method}
% In this section, we propose a novel Bayesian imitation learning framework which learns policy and a inject noise distribution simultaneously using multi-modal policy model based on IOMGP \cite{ross2013nonparametric}.
% % For simplicity, but without loss of generality, in this section, we focus on one-dimensional action variable.

% \subsection{Policy Model}
% In order to learn a multi-modal policy, we assume infinite multi-modal GP for policy prior as:
% \begin{align}
%     \pi \sim \prod_{m=1}^{\infty} \mathcal{GP}^{(m)} \left(\mathbf{0}, \mathbf{k}^{(m)}(\mathbf{s}, \mathbf{s}^{\prime})\right),
% \end{align}
% where $\mathrm k^{(m)}(\cdot,\cdot)$ is kernel function for $m$-th GP.

% 潜在変数$\mathbf f^{(m)}$の事前分布
% \begin{equation}\label{prior_GP}
%     p(\{\mathbf{f}^{(m)}\} \mid\mathbf{S})=\prod_{m=1}^{\infty}  \mathcal{N}(\mathbf{f}^{(m)} \mid\mathbf{0},\mathbf{K}^{(m)}; \boldsymbol{\omega}^{(m)})
% \end{equation}

% \begin{align}
%     \label{prior_z}
%     p(\mathbf{Z} \mid \mathbf{v}) &= \prod_{n=1}^{N} \prod_{m=1}^{\infty}\left(v_{m} \prod_{j=1}^{m-1}\left(1-v_{j}\right)\right)^{\mathbf{Z}_{nm}} \\
%     \label{prior_v}
%     p(\mathbf{v} \mid \alpha) &= \prod_{m=1}^{\infty} \operatorname{Beta}\left(v_{m} \relmiddle| 1,\alpha\right)
% \end{align}

% \begin{align}\label{MGP-DART:likelihood}
%     &p(\mathbf a^*\mid\{\mathbf f^{(m)}\},\mathbf f^{(m)}, \mathbf{Z}; \{{\sigma}_{k+1}^2\}) \nonumber\\
%     &=\prod^{k}_{j=1} \prod^{N_j}_{n=N_{j-1}} \prod^{\infty}_{m=1}
%     \left[ \mathcal{N}\left(a^*_n \relmiddle| \mathbf{f}_{n}^{k(m)} , \sigma_{j+1}^2\right)\right]^{\mathbf{Z}_{n, m}}\nonumber\\
%     &=\prod_{n=1}^{N}\prod_{m=1}^{\infty} \mathcal{N}(\mathbf{a}_n^*\mid \mathbf{f}_n^{k(m)},\Sigma_{n, n})^{\mathbf{Z}_{n, m}}
% \end{align}

% where, $\{\sigma_{k+1}^2\}$, $\Sigma$ is :
% \begin{equation}\label{MGP:variance_set}
%     \{\sigma_{k+1}^2\}=\{\sigma_2^2,\sigma_3^2, \cdots, \sigma_{k+1}^2\}
% \end{equation}
% \begin{equation}
%     \Sigma = 
%         \begin{bmatrix}
%         \sigma_2^2 \mathbf{I}_{T}  & 0 & \cdots & 0\\
%          0& \sigma_3^2 \mathbf{I}_{T} & \cdots & 0\\
%         \vdots  & \vdots & \ddots & \vdots \\
%         0  & 0 & \cdots & \sigma_{k+1}^2 \mathbf{I}_{T}
%         \end{bmatrix}
% \end{equation}
% \color{black}
%============================================================================

\section{Proposed method}
In this section, we propose a novel Bayesian imitation learning framework (Fig. \ref{fig:concept}) which learns a multi-modal policy by an expert demonstration with noise injection.
We employ IOMGP \cite{ross2013nonparametric} as a policy prior and incorporate the injected noise distribution as a likelihood to a policy model.
We derive an imitation learning method which learns a multi-modal policy and a injected noise distribution by variational Bayesian learning.


% \color{red}
% \subsection{Policy Model}
% To learn multimodal policy, we consider the policy prior as the following product of infinite GPs:
% \begin{equation}
%     {\pi} \sim \prod_{m=1}^{\infty} \mathcal{GP}^{(m)} \left(\mathbf{0}, \mathrm{k}^{(m)}(\mathbf{s}, \mathbf{s}^{\prime})\right).
% \end{equation}
% where $\mathrm{k}^{(m)}(\cdot,\cdot)$ is kernel function for $m$-th GP, and $\mathbf s$ is an input for a policy.
% 
% We define the following priors for the collected data by $k$-th iteration 
% \begin{align}\label{prior_GP}
%     p(\{\mathbf{f}^{(m)}\} \mid\mathbf{S}) &= \prod_{m=1}^{\infty}  p(\mathbf f^{(m)}\mid \mathbf S) \\
%     p(\mathbf f^{(m)}\mid \mathbf S) &= \mathcal{N}(\mathbf{f}^{(m)} \mid\mathbf{0},\mathbf{K}^{(m)}; \omega^{(m)})
% \end{align}
% where $\mathbf{K}^{(m)}=\mathrm{k}^{(m)}({\mathbf{S}}, {\mathbf{S}})$ is the $m$~th kernel gram matrix with a kernel hyperparameter $\omega^{(m)}$.
% 
% \begin{align}\label{prior_z}
%     p(\mathbf{Z} \mid \mathbf{v}) &= \prod_{n=1}^{N} \prod_{m=1}^{\infty}\left(v_{m} \prod_{j=1}^{m-1}(1-v_{j})\right)^{\mathbf{Z}_{nm}} \\
%     p(\mathbf{v} \mid \alpha)&=\prod_{m=1}^\infty \operatorname{Beta}(v_{m} \mid 1,\alpha)
% \end{align}
% 
% \begin{align}\label{MGP-DART:likelihood}
%     p({\mathbf{a}^*} \mid\{\mathbf{f}^{(m)}\}, \mathbf{Z}; \{{\sigma}_{k}^2\})=\prod_{n=1}^{N}\prod_{m=1}^{\infty} \mathcal{N}(\mathbf{a}_n^*\mid \mathbf{f}_n^{(m)},\boldsymbol\Sigma_{nn})^{\mathbf{Z}_{nm}}
% \end{align}
% where, $\boldsymbol\Sigma=\mathrm{diag}\{\sigma_i\mathbf 1_{N_i}\}_{i=1}^k$, $\mathbf 1_{N_i}$ is a vector whose size is $N_i$ and all components are one.
% 
% 
% \color{black}

\subsection{Policy Model}
To learn multimodal policy, we consider the policy prior as the following product of infinite GPs:
\begin{equation}
    {\pi} \sim \prod_{m=1}^{\infty} \mathcal{GP}^{(m)} \left(\mathbf{0}, \mathrm{k}^{(m)}(\mathbf{s}, \mathbf{s}^{\prime})\right)
\end{equation}
where $\mathrm{k}^{(m)}(\cdot,\cdot)$ is kernel function for $m$-th GP.
Considering $m$-th GP's output as a latent function $\mathbf{f}^{(m)}$, and prepare an indicator matrix $\Z$ that shows the association between each state-action pair of training data and a latent function $\mathbf{f}^{(m)}$.
Also, $k$ injection noise parameters $\{{\sigma}_{k+1}^2\} = \{\sigma_{j+1}^2\}_{j=1}^{k}$ are defined to associate the training data collected in the $k$~th iteration with the injection noise parameter.
These are provide a probabilistic measure for infer the multimodal policies
and optimizing the injection noise parameter in the follow iteration.

The training dataset collected by the noise injected expert through the $k$~th iteration is defined as $\mathcal{D}=[\mathbf{a^*},\mathbf{S}]$, where $\mathbf{S}=[\mathbf{s}_n]_{n=1}^{N}$ and $\mathbf{a^*}=[a^*_n]_{n=1}^{N}$ represent series of $N = \sum_{j=1}^{k} N_j$ state-action pairs, $N_j$ is a size of the dataset that collected at $j$~th iteration.
We denote the set of latent functions with $\{ {\mathbf{f}}^{(m)}\}=\left\{\mathbf{f}^{(m)}(\mathbf{S}) \right\}^{\infty}_{m=1}$ and the prior distribution is given by :

\begin{equation}\label{prior_GP}
    p(\{\mathbf{f}^{(m)}\} \mid\mathbf{S}, \{\boldsymbol\omega^{(m)}\})=\prod_{m=1}^{\infty}  \mathcal{N}(\mathbf{f}^{(m)} \mid\mathbf{0},\mathbf{K}^{(m)}; \omega^{(m)})
\end{equation}
where $\mathbf{K}^{(m)}=\mathrm{k}^{(m)}({\mathbf{S}}, {\mathbf{S}})$ is the $m$~th kernel gram matrix with a kernel hyperparameter $\omega^{(m)}$.
Let $\{\boldsymbol{\omega}^{(m)}\} = \{\omega^{(m)}\}^{\infty}_{m=1}$ be the set of hyperparameters of infinite number of kernel functions.

Then place the Stick Breaking Process (SBP) \cite{sethuraman1994constructive} as the prior distribution of $\Z$, which can be interpreted as an infinite mixture model as follows:
\begin{align}\label{prior_z}
    p(\mathbf{Z} \mid \mathbf{v}) &= \prod_{n=1}^{N} \prod_{m=1}^{\infty}\left(v_{m} \prod_{j=1}^{m-1}\left(1-v_{j}\right)\right)^{\mathbf{Z}_{nm}} \\
    p(\mathbf{v} \mid \alpha)&=\prod_{m=1}^{\infty} \operatorname{Beta}\left(v_{m} \relmiddle| 1,\alpha\right)
\end{align}

Note that the implementation of variational Bayesian learning cannot deal with infinite-dimensional vectors, so we replace the $\infty$ component with a predefined upper bound of the mixtures $M$.
${{v}_m}$ is a random variable indicating the probability that the data corresponds to the $m$~th GP, and $\alpha$ is a hyperparameter of SBP denoting the level of concentration of the data in the cluster.

To learn the policy and injection noise parameters simultaneously in the same framework, we derive a likelihood function by integrating the likelihood function of the learned policy (\ref{DART:Noise}) with a likelihood function that explains the training data's actions with latent variables $\F,\Z$.

The optimization of the policy is performed using all the training data collected up to k iteration.
In contrast, the optimization of the injection noise parameters (\ref{DART:Noise}) deals with the training data collected in a $k$~th iteration.
To integrate the two optimization problems into one, it is necessary to define new injection noise parameters at iteration start-up and correspond to the training data collected from iteration.
Thus, we define heteroscedastic Gaussian noise and indicate the association between the training dataset collected for each iteration and the injection noise parameters as:
\begin{equation}
    \boldsymbol\Sigma=\mathrm{diag}\{\sigma_i\mathbf 1_{N_i}\}_{i=1}^k 
\end{equation}
where, $\mathbf 1_{N_i}$ is a vector whose size is $N_i$ and all components are one.
It provides a framework to leverage the overall data to optimize the injection noise parameter.
Using the fact that the value of the likelihood (\ref{DART:Noise}) does not change even if the mean and the input of the likelihood are replaced.
Therefore, the likelihood for the  $\{\mathbf{f}^{(m)}\}, \mathbf{Z}, \{{\sigma}_{k+1}^2\} $ is derived as :
% \begin{align}\label{MGP-DART:likelihood}
%     & p\left({\mathbf{a}^*} \relmiddle|\{\mathbf{f}^{(m)}\}, \mathbf{Z}; \{{\sigma}_{k}^2\} \right) \nonumber\\
%     &=\prod^{k}_{j=1} \prod^{N_j}_{n=N_{j-1}} \prod^{\infty}_{m=1}
%     \left[ \mathcal{N}\left(a^*_n \relmiddle| \mathbf{f}_{n}^{(m)} , \sigma_{j+1}^2\right)\right]^{\mathbf{Z}_{n, m}}\nonumber\\
%     &=\prod_{n=1}^{N_k}\prod_{m=1}^{\infty} \mathcal{N}({a}_n^*\mid \mathbf{f}_n^{(m)},\Sigma_{n, n})^{\mathbf{Z}_{n, m}}
% \end{align}
\begin{align}\label{MGP-DART:likelihood}
    p({\mathbf{a}^*} \mid\{\mathbf{f}^{(m)}\}, \mathbf{Z}; \{{\sigma}_{k+1}^2\} ) 
    % &=\prod^{k}_{j=1} \left[ \prod^{N_j}_{n=1} \prod^{\infty}_{m=1}
    %  \mathcal{N}\left(a_n^{j*} \relmiddle| \mathbf{f}_{t}^{j(m)} , \sigma_{j+1}^2\right)^{\mathbf{Z}_{n, m}}\right]\nonumber\\
        =\prod_{n=1}^{N}\prod_{m=1}^{\infty} \mathcal{N}({a}_n^*\mid \mathbf{f}_n^{(m)},\Sigma_{nn})^{\mathbf{Z}_{nm}}
\end{align}

% where,$\Sigma$ is :

% \begin{equation}
%     \Sigma = 
%         \begin{bmatrix}
%         \sigma_1^2 \mathbf{I}_{N_1}  & 0 & \cdots & 0\\
%          0& \sigma_2^2 \mathbf{I}_{N_2} & \cdots & 0\\
%         \vdots  & \vdots & \ddots & \vdots \\
%         0  & 0 & \cdots & \sigma_{k}^2 \mathbf{I}_{N_{k}}
%         \end{bmatrix}
% \end{equation}

% Therefore, the likelihood conditional on $\{\mathbf{f}^{(m)}\},\mathbf{Z}$ as : 
% \begin{equation}\label{MGP-DART:likelihood}
%     p\left({\mathbf{a}^*} \relmiddle|\{\mathbf{f}^{(m)}\}, \mathbf{Z}; \{{\sigma}_{k+1}^2\} \right) =
%     \prod_{n=1}^{N}\prod_{m=1}^{\infty} \mathcal{N}\left({\mathbf{a}_n^*} \relmiddle| \mathbf{f}_n^{(m)}, \Sigma \right)^{\mathbf{Z}_{n, m}}
% \end{equation}


We can describe such a formulation in a graphical model that defines the relationship between the variables as shown in Fig.~\ref{fig:concept}, and the joint distribution of the model as :
\begin{align}\label{joint_distribution}
    &p({\mathbf{a}^*}, \mathbf{Z}, \mathbf{v},\{\mathbf{f}^{(m)}\}\mid\mathbf{S} ;\Omega ) \nonumber\\
    &=p({\mathbf{a}^*} \mid\{\mathbf{f}^{(m)}\}, \mathbf{Z}; \{{\sigma}_{k+1}^2\})\cdot \nonumber\\
    &~~~~~~~~p(\{\mathbf{f}^{(m)}\} \mid\mathbf{S}; \{\boldsymbol{\omega}^{(m)}\})
    p(\mathbf{Z} \mid \mathbf{v}) p(\mathbf{v} \mid \alpha)
\end{align}
where $\Omega =(\{\boldsymbol{\omega}^{(m)}\},\{{\sigma}_{k+1}^2\},\alpha)$ represents a set of hyperparameters.
% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=\hsize]{Figure/Generative_model.pdf}
%     \caption{Graphical model of MGP-DART}
%     \label{fig:generative_model}
% \end{figure}


==> sections/experiments_v1.tex <==
\section{EXPERIMENT}
%--------------------------------------------------------------------------------
The objective of this paper is to develop robust and flexible imitation learning.
In this regard, we have prepared an experiment to answer the following questions.
\romannumeral 1) Does MGP-DART learn policies with multiple optimal behaviors (flexibility)?
\romannumeral 2) Can MGP-DART reduce covariate shift (robustness)?
\romannumeral 3) Does MGP-DART induce excessive noise (which can be a serious challenge for supervisors) injection due to modeling errors like DART\cite{laskey2017dart}?

We compared proposed method (MGP-DART) with DART using standard unimodal GPs (UGP-DART), BC using infinite overlapping mixtures of Gaussian processes (MGP-BC) and BC using standard unimodal GPs (UGP-BC).
Note the parameter M (i.e. Maximum number of mixtures of GPs) is set to an appropriate value (M = 5) throughout the experiment to avoid the limitation of the flexibility of the policy model (if $M$ is too small) and the high computational complexity (if $M$ is too large).
With regard to \romannumeral 3) we confirmed the degree of variability of the noise parameters (the variance of the noise distribution) of MGP-DART and UGP-DART via optimization.

\subsection{With Simulation}
We have constructed two tasks: 1) push and place task, and 2) table-sweep task with simulation.
Both tasks have multi-target objects to validate the flexibility
and include the motion of pushing an object to verify robustness.
This motion leads to a large deviation in the direction and distance of the object's draft due to the friction between objects, table, and robot's gripper.
Thus if the initial condition (position of each object) changes even slightly, the learned policy in standard BC tends to have a large covariate shift.

\subsubsection{Push and Place Task}
\begin{figure}
    \centering
    \includegraphics[width =\hsize]{Figure/Mujoco/Mujoco_push.pdf}
    \vspace{-2mm}
    \caption{MuJoCo environment used in the experiment. The state is the position of objects placed on the table and the action is the velocity at which the robot arm is moved.}
    \label{fig:Mujoco_env}
\end{figure}
An initial experiment was conducted by training a push and place task in the MuJoCo~\cite{todorov2012mujoco} environment as shown in Fig.~\ref{fig:Mujoco_env} to verify the ability of MGP-DART to learn a probabilistic policy that has multi optimal actions and reduce the covariate shift.

% Task setup
The goal of the task is to make the robot arm push a black box on the table to the goal(★) shown in the Fig.~\ref{fig:Mujoco_env}.
% Data collecting and Training
With two goals on the table, a robot trajectory steered by an algorithmic supervisor to make an box reach one of the goals is considered to be one demonstration.
Where an algorithmic supervisor is a velocity controller for a robot arm using a classical PID controller \cite{sellers2001pid}.

After collecting two demonstration data sets that reach both goals, we optimize the policy and noise parameters until (\ref{MGP:objective_function}) is converged.
From the collection of the two demonstrations to the optimization of the policy and noise parameters in one iteration, we performed 10 iterations.
The maximum number of iterations was determined based on the convergence of the noise parameters.

We denote the states are the x,y position of two goals and a box on the table and the robot arm (in 8 dimensions), and the action is the velocity of the robotic arm (in 2 dimensions).

To validate the performance of MGP-DART in reducing covariate shift, the initial positions of the robot arm and the black box were randomly placed to induce scenarios in which covariate shift tended to be large during the test episodes.

The performance of MGP-DART was compared by rewarding whether or not the black box was placed in the goal at the end of the test episode (False : 0, True : 1).



\subsubsection{Table-sweep Task}
\begin{figure}
    \centering
    \includegraphics[width =0.7\hsize]{Figure/V-REP/V-REP.pdf}
    \vspace{-2mm}
    \caption{V-REP environment used in the experiment of table-sweep task. The state is the position of objects placed on the table and the action is the velocity at which the robot arm is moved.}
    \label{fig:V-REPenv}
\end{figure}
The following experiments were conducted to confirm the scalability as well as the learning of probabilistic policy and the reduction of covariate shift by applying MGP-DART to a more complex task (i.e. table-sweep task) sweeping three boxes on a table in a V-Rep environment as shown in the Fig.~\ref{fig:V-REPenv}.

The goal of this task is for the robot arm to sweep the boxes out of the table to create a work-space on the table.
The algorithmic supervisor is a velocity controller of the robot arm using a classical PID controller as well as a push and place task \cite{sellers2001pid}.
Let one demonstration describe the trajectory of a robot controlled by an algorithmic supervisor, which sweeps all the boxes out of the table in order.

After placing the boxes on the table in an arbitrary array and collecting three demonstration data sets that sweep in random order, we optimize the policy and noise parameters until \ref{MGP:objective_function} is converged.

From the collection of the three demonstrations to the optimization of the policy and noise parameters in one iteration, we performed 10 iterations.
The maximum number of iterations was determined based on the convergence of the noise parameters.

% Task setup
The state in the task is the relative coordinate between the robot arm and the three boxes (in 6 dimensions), and
Action is defined as the velocity of the robot arm in the x and y axis.

To validate the performance of MGP-DART in reducing covariate shift, 
the initial positions of three boxes were randomly placed on the table to induce scenarios in which covariate shift tended to be large during the test episodes.
The performance of learning models was calculated as a reward for the total number of boxes out of the table at the end of the test episode (Min : 0, Max : 3).

\subsection{With Real robot}
\begin{figure}
    \centering
    \includegraphics[width =0.7\hsize]{Figure/Realrobot/env.pdf}
    \vspace{-2mm}
    \caption{Experimental environment for Real robot(UR3) table-sweep task. The state is the position of objects placed on the table and the action is the velocity at which the robot arm is moved.}
    \label{fig:Realenv}
\end{figure}
A final experiment, MGP-DART with the human supervisor was utilized to verify the UR3 robot can learn the task to create a workspace by sweeping office supplies (i.e. rubber tape, etc.) placed on the table as shown in Fig.~\ref{fig:Realenv}. 

The goal of this task is a robot arm sweeps the office supplies out of the table.
A demonstration is a trajectory in which a robot controlled by a human supervisor sweeps all the office supplies out of the table in order.

Before each demonstration begins, the two objects are arbitrarily placed in a circle on the table, and the human supervisor controlling the robotic arm collects two demonstrations in which each office supply is swept off the table in random order and then optimizes the measure and the noise parameter until (18) is converged.
The process from the collection of two demonstration datasets to the optimization of policy and noise parameters was repeated 5 times.

For the state of the experiment, the x,y position was obtained by recognizing AR markers attached to each object (robot arm and rubber tape) through a camera, and the x,y velocity of the UR3 robot arm was placed in the action.

To validate the performance of MGP-DART in reducing covariate shift, 
the initial positions of office supplies were arbitrarily placed in a circle on the table to induce scenarios in which covariate shift tended to be large during the test episodes.
The performance of learning models was calculated as a reward for the total number of boxes out of the table at the end of the test episode (Min : 0, Max : 2).
\clearpage

==> sections/experiments_v2.tex <==
\section{EVALUATION}
%--------------------------------------------------------------------------------
In this section, the proposed approach is evaluated through simulation and experiments on a 7DOF robotic manipulator. Specifically, to evaluate the robustness and flexibility of the proposed approach, the following key questions are investigated:
\romannumeral 1) Can MGP-DART learn policies with multiple optimal behaviors, thereby retaining flexibility?
\romannumeral 2) Can MGP-DART reduce covariate shift error, thereby improving model robustness?
\romannumeral 3) Is the noise induced by MGP-DART of significantly low variance, allowing for safe perturbed demonstrations?


%induce excessive noise (which can be a serious challenge for supervisors) injection due to modeling errors like DART\cite{laskey2017dart}?
\begin{table}[]
\centering
\begin{tabular}{l|cc}
\hline
                  & Flexibility    & Robustness     \\ \hline\hline
UGP-BC   & $-$    & $-$    \\ \hline
UGP-DART & $-$    & $\checkmark$ \\ \hline
MGP-BC   & $\checkmark$ & $-$    \\ \hline
MGP-DART & $\checkmark$ & $\checkmark$ \\ \hline
\end{tabular}
\caption{Comparing models without flexibility or robustness to validate the effectiveness of the proposed method of balancing flexibility and robustness.}
\label{table:model}
\end{table}

To evaluate the proposed method (MGP-DART), comparisons against naive policy learning methods as TABLE~\ref{table:model}, including:
\begin{inparaenum}
\item BC using standard unimodal GPs (UGP-BC) \cite{rasmussen2003gaussian} ,
\item DART using standard unimodal GPs (UGP-DART) ,
\item BC using infinite overlapping mixtures of Gaussian processes (MGP-BC) , and
\end{inparaenum}

Specifically, these three are chosen due to their [...].

In all applications of these methods, the maximum number of mixture GPs is fixed at ($M = 5$). This value is selected through cross-validation on reported accuracy. It is a reasonable trade-off between limiting the flexibility of the policy model (if $M$ is too small) and the high computational complexity (if $M$ is too large).

About \romannumeral 3), we confirmed the degree of variability of the noise parameters (the variance of the noise distribution) of MGP-DART and UGP-DART via optimization.

\subsection{Simulation}
%The goal of this first evaluation is to [...]

The first evaluation aims to characterize the flexibility and robustness of the proposed approach for learning and completing tasks in a complex environment.  Specifically, two standard manipulator learning tasks involving object manipulation are presented: 
\begin{inparaenum}
\item push and place, and
\item table-sweeping.
\end{inparaenum}

These tasks are well suited to evaluating the learned-policy in terms of:
\begin{inparaenum}
\item flexibility, due to the presence of multi-optimal targets and objects in the scene, and
\item robustness, environmental factors, such as friction between objects, tables, and robot grippers, cause environmental variations in object position and movement. Thus if the initial condition (position of each object) changes slightly, the learned policy in standard BC tends to have a large covariate shift.
\end{inparaenum}

%Both tasks have multi-target objects to validate the flexibility and include the motion of pushing an object to verify robustness.

%This motion leads to a large 


\subsubsection{Push and Place Task}
\begin{figure}
    \centering
    \includegraphics[width =0.4\hsize]{Figure/Mujoco/Mujoco_env.pdf}
    \vspace{-2mm}
    \caption{MuJoCo environment used in the experiment. The state is the position of objects placed on the table and the action is the velocity at which the robot arm is moved.}
    \label{fig:Mujoco_env}
\end{figure}
An initial experiment is conducted by training a push and place task in the MuJoCo~\cite{todorov2012mujoco} environment as shown in the Fig.~\ref{fig:Mujoco_env}, to verify the ability of MGP-DART to learn a probabilistic policy that has multi optimal actions, thereby limiting the covariate shift.

% Task setup
This task aims to teach the robotic arm to push the black box on the table to either of the goal positions (★), as shown in Fig.~\ref{fig:Mujoco_env}.
% Data collecting and Training
For this, demonstrations are first generated by an expert demonstrator. For this simulation, a simple algorithmic supervisor (a velocity controller for a robot arm using a classical PID controller \cite{sellers2001pid}) is used to move to either of the two-goal positions. The state of the system is defined as the coordinates of both goals and the box on the table. The joint configuration of the robot arm (in 8 dimensions), and the action is the velocity of the robotic arm (in 2 dimensions).

\begin{algorithm}[tb]
\caption{BM: Notes for data collection and learning}
\label{algorithm_pushandplace_experiment_overview}
\begin{algorithmic}[1]
% \small
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE %$M,K,T$
\ENSURE %{$q,\hat{\Omega}$}
\FOR {Experiments = {1..5}}
    \STATE Empty Dataset defined
    \FOR {Policy iterations = {1..10}}
        \STATE Demonstrator moves the box to state 1
        \STATE Demonstrator moves the box to state 2
        \STATE Demonstrations appended to Dataset
        \STATE MGP-DART optimizes noise and policy on Dataset
    \ENDFOR
\ENDFOR
\end{algorithmic} 
\end{algorithm}

%The data collection and optimization procedure is outlined in (\ref{algorithm_pushandplace_experiment_overview}), following the standard imitation learning procedure. 

The data collection and optimization procedure is outlined as follows. Firstly, the Demonstrator performs two push and place actions (one for each goal position). Using these two demonstrations the policy and noise parameters are optimized until (\ref{MGP:objective_function}) reaches convergence. This procedure is repeated for ten iterations, continuously updating the policy and noise given these additional demonstrations. The maximum number of iterations is determined based on the convergence of the noise parameters. $N=5$ independent repeats of this experiment are performed to evaluate the robustness of the approach. The robot arm's initial position and the black box were randomly placed to induce scenarios in which the covariate shift tended to be large. For each evaluation of the methods, a reward is given if the black box was placed in the goal at the end of the test episode (False : 0, True: 1).

\subsubsection{Table-sweep Task}
\begin{figure}
    \centering
    \includegraphics[width =0.7\hsize]{Figure/V-REP/VREP_env.pdf}
    \vspace{-2mm}
    \caption{V-REP environment used in the experiment of the table-sweep task. The state is the position of objects placed on the table, and the action is the velocity at which the robot arm is moved.}
    \label{fig:V-REPenv}
\end{figure}
In addition to the push-and-place task, and the table-sweep task is also performed to evaluate the scalability of the proposed approach to a more complex task. In this, boxes are placed at random coordinates on a table, and are then swept off by the manipulator in a V-Rep environment, as shown in the Fig.~\ref{fig:V-REPenv}. Demonstrations are generated using a PID controller \cite{sellers2001pid}, similarly to the push-and-place task. A successful demonstration is defined as the manipulator sweeping away all blocks. The data collection and optimization procedure is similar to the push-and-place task, whereby after a successful demonstration, the policy and noise parameters are optimized until \ref{MGP:objective_function} converges. This procedure is repeated for 10 iterations, continuously updating the policy and noise estimates.

%Similarly to the push-and-place task, the algorithmic supervisor is a velocity controller of the robot arm using a classical PID controller as well as a push and place task \cite{sellers2001pid}.

%A demonstration describe the trajectory of a robot controlled by an algorithmic supervisor, which sweeps all the boxes out of the table in order.

%as well as the learning of probabilistic policy and the reduction of covariate shift by applying MGP-DART  sweeping three boxes on a table in a V-Rep environment as shown in the Fig.~\ref{fig:V-REPenv}.

%The goal of this task is for the robot arm to sweep the boxes out of the table to create a work-space on the table.

%After placing the boxes on the table in an arbitrary array and collecting three demonstration data sets that sweep in random order, 

%From the collection of the three demonstrations to the optimization of the policy and noise parameters in one iteration, we performed 10 iterations.
%The maximum number of iterations was determined based on the convergence of the noise parameters.

% Task setup
The task's state is the relative coordinate between the robot arm and three boxes (in 6 dimensions). An action is defined as the velocity of the robot arm in the x and y axis.

To validate the performance of MGP-DART in reducing covariate shift, 
the initial positions of three boxes were randomly placed on the table to induce scenarios in which the covariate shift tended to be large during the test episodes.
The learning models' performance was calculated as a reward for the total number of boxes out of the table at the end of the test episode (Min : 0, Max : 3).

\subsection{UR3 Manipulator}
\begin{figure}
    \centering
    % \includegraphics[width =0.7\hsize]{Figure/Realrobot/env.pdf}
    \includegraphics[width =0.7\hsize]{Figure/Realrobot/env2.pdf}
    \vspace{-2mm}
    \caption{Experimental environment for Real robot(UR3) table-sweep task. The state is the position of objects placed on the table and the action is the velocity at which the robot arm is moved.}
    \label{fig:Realenv}
\end{figure}
A final experiment, MGP-DART with the human supervisor was utilized to verify the UR3 robot can learn the task to create a workspace by sweeping office supplies (i.e. rubber tape, etc.) placed on the table as shown in Fig.~\ref{fig:Realenv}. 

The goal of this task is a robot arm sweeps the office supplies out of the table. A demonstration is a trajectory in which a robot controlled by a human expert sweeps all the office supplies out of the table in order.

Before each demonstration begins, the two objects are arbitrarily placed in a circle on the table, and the human expert controlling the robotic arm collects two demonstrations in which each office supply is swept off the table in random order and then optimizes the measure and the noise parameter until (18) is converged.
The process from collecting two demonstration datasets to the optimization of policy and noise parameters was repeated five times.

For the experiment's state, the x,y position was obtained by recognizing AR markers attached to each object (robot arm and rubber tape) through a camera. The x,y velocity of the UR3 robot arm was placed in the action.

To validate the performance of MGP-DART in reducing covariate shift, 
the initial positions of office supplies were arbitrarily placed in a circle on the table to induce scenarios in which the covariate shift tended to be large during the test episodes.
The learning models' performance was calculated as a reward for the total number of boxes out of the table at the end of the test episode (Min : 0, Max: 2).
%\clearpage

==> sections/experiments_v3.tex <==
\begin{figure*}[tb]
    \centering
    % \includegraphics[width =\hsize]{Figure/V-REP/VREP-ex.pdf}
    % \includegraphics[width =0.7\hsize]{Figure/V-REP/VREP-ex_v2.pdf}
    % \includegraphics[width =0.9\hsize]{Figure/V-REP/VREP-ex_v3.pdf}
    \includegraphics[width =0.9\hsize]{Figure/V-REP/VREP-ex_v4.pdf}
    \vspace{-2mm}
    \caption{
    (a) V-REP environment used in the experiment of the table-sweep task. The task's state is the relative coordinate between the robot arm and boxes. An action is defined as the velocity of the robot arm in the x and y axis.
    \textbf{Flexibility}:
    (b) is a plot of stochastic policies for the MGP and the UGP policy model in the task's starting state.
    Since the UGP policy model has a unimodal distribution of actions, it outputs actions that pass through the middle of the two boxes, as shown in (c). 
    In contrast, the MGP policy model has a multimodal distribution and can output the optimal action that sweeps each of the two boxes, as shown in (c).
    \textbf{Robustness}:
    (d) is a plot of the predicted action variance through MGP-DART and MGP-BC for each step of the test.
    (e) When the robot contacts the box and initiates a sweep, the MGP-BC tends to increase uncertainty and fails the task. MGP-DART, however, tends to take actions that reduce uncertainty and can succeed in the task.
    }
    \label{fig:V-REP}
\end{figure*}

\section{EVALUATION}
%--------------------------------------------------------------------------------
In this section, the proposed approach is evaluated through simulation and experiments on a 7DOF robotic manipulator. Specifically, to evaluate the robustness and flexibility of the proposed approach, the following key questions are investigated:
\romannumeral 1) Can MGP-DART learn policies with multiple optimal behaviors, thereby retaining flexibility?
\romannumeral 2) Can MGP-DART reduce covariate shift error, thereby improving model robustness?
\romannumeral 3) Is the noise induced by MGP-DART of significantly low variance, allowing for safe perturbed demonstrations?


%induce excessive noise (which can be a serious challenge for supervisors) injection due to modeling errors like DART\cite{laskey2017dart}?
\begin{table}[]
\centering
\begin{tabular}{l|cc}
\hline
                  & Flexibility    & Robustness     \\ \hline\hline
UGP-BC   & $-$    & $-$    \\ \hline
UGP-DART & $-$    & $\checkmark$ \\ \hline
MGP-BC   & $\checkmark$ & $-$    \\ \hline
MGP-DART & $\checkmark$ & $\checkmark$ \\ \hline
\end{tabular}
\caption{Comparing models without flexibility or robustness to validate the effectiveness of the proposed method of balancing flexibility and robustness.}
\label{table:model}
\end{table}

To evaluate the proposed method (MGP-DART), comparisons against naive policy learning methods, including:
\begin{inparaenum}
\item Imitation learning with supervised learning (\ie Behavior Cloning (BC)\cite{bain1995framework}) using standard unimodal GPs (UGP-BC) \cite{rasmussen2003gaussian},
\item DART using standard unimodal GPs (UGP-DART),
\item BC using infinite overlapping mixtures of Gaussian processes (MGP-BC).
\end{inparaenum}
Specifically, these three are chosen due to their lack of flexibility and robustness as TABLE~\ref{table:model}.

In all applications of these methods, the maximum number of mixture GPs is fixed at ($M = 5$). This value is selected through cross-validation on reported accuracy. It is a reasonable trade-off between limiting the flexibility of the policy model (if $M$ is too small) and the high computational complexity (if $M$ is too large).

About \romannumeral 3), we confirmed the degree of variability of the noise parameters (the variance of the noise distribution) of MGP-DART and UGP-DART via optimization.

%The goal of this first evaluation is to [...]
\subsection{Simulation}
The first evaluation aims to characterize the flexibility and robustness of the proposed approach for learning and completing tasks in a complex environment.  Specifically, standard manipulator learning task (\ie table-sweep task) involving object manipulation are presented.

These tasks are well suited to evaluating the learned-policy in terms of:
\begin{inparaenum}
\item flexibility, due to the presence of multi-optimal targets and objects in the scene, and
\item robustness, environmental factors, such as friction between objects, tables, and robot grippers, cause environmental variations in object position and movement. Thus if the initial condition (position of each object) changes slightly, the learned policy in standard BC tends to have a large covariate shift.
\end{inparaenum}

%Both tasks have multi-target objects to validate the flexibility and include the motion of pushing an object to verify robustness.

%This motion leads to a large 

\begin{figure}
    \centering
    % \includegraphics[width =\hsize]{Figure/V-REP/Result_v1.pdf}
    \includegraphics[width =\hsize]{Figure/V-REP/Result_v2.pdf}
    \caption{The mean and standard deviation of the rewards of 100 tests of each of the four models, MGP-DART and UGP-DART, MGP-BC and UGP-BC.The change in the variance of the noise by optimizing the noise parameters (variance) of MGP-DART and UGP-DART}
    \label{fig:performance}
\end{figure}

% introduction of table sweep task with 2 target objects
% motivation of experiment
% environment / task setup
% Learning overview
% - how to collect training data
% - 
An initial experiment is conducted by training a table-sweep task in the V-REP~\cite{rohmer2013VREP} environment as shown in the Fig.~\ref{fig:V-REP}-(a), to verify the ability of MGP-DART to learn a probabilistic policy that has multi optimal actions, thereby limiting the covariate shift.

In this, boxes are placed at fixed coordinates on a table, and are then swept off by the manipulator in a V-Rep environment, as shown in the Fig.~\ref{fig:V-REP}. Demonstrations are generated using a PID controller \cite{sellers2001pid}. A successful demonstration is defined as the manipulator sweeping away all blocks. The data collection and optimization procedure is after a successful demonstration, the policy and noise parameters are optimized until (\ref{MGP:objective_function}) converges. This procedure is repeated for 10 iterations, continuously updating the policy and noise estimates.

% \begin{algorithm}[tb]
% \caption{Notes for data collection and learning}
% \label{algorithm_pushandplace_experiment_overview}
% \begin{algorithmic}[1]
% % \small
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \REQUIRE %$M,K,T$
% \ENSURE %{$q,\hat{\Omega}$}
% \FOR {Experiments = {1..5}}
%     \STATE Empty Dataset defined
%     \FOR {Policy iterations = {1..10}}
%         \STATE Demonstrator moves the box to state 1
%         \STATE Demonstrator moves the box to state 2
%         \STATE Demonstrations appended to Dataset
%         \STATE MGP-DART optimizes noise and policy on Dataset
%     \ENDFOR
% \ENDFOR
% \end{algorithmic} 
% \end{algorithm}

%The data collection and optimization procedure is outlined in (\ref{algorithm_pushandplace_experiment_overview}), following the standard imitation learning procedure. 

The data collection and optimization procedure is outlined as follows. Firstly, the Demonstrator performs two push and place actions (one for each goal position). Using these two demonstrations the policy and noise parameters are optimized until (\ref{MGP:objective_function}) reaches convergence. This procedure is repeated for ten iterations, continuously updating the policy and noise given these additional demonstrations. The maximum number of iterations is determined based on the convergence of the noise parameters. $N=5$ independent repeats of this experiment are performed to evaluate the robustness of the approach. The robot arm's initial position and the black box were randomly placed to induce scenarios in which the covariate shift tended to be large. For each evaluation of the methods, a reward is given if the black box was placed in the goal at the end of the test episode (False : 0, True: 1).

\subsubsection{Table-sweep Task}

% \begin{figure}
%     \centering
%     \includegraphics[width =0.5\hsize]{Figure/V-REP/VREP_env_UP.pdf}
%     \vspace{-2mm}
%     \caption{V-REP environment used in the experiment of the table-sweep task. The state is the position of objects placed on the table, and the action is the velocity at which the robot arm is moved.}
%     \label{fig:V-REPenv}
% \end{figure}
In addition to the push-and-place task, and the table-sweep task is also performed to evaluate the scalability of the proposed approach to a more complex task. In this, boxes are placed at random coordinates on a table, and are then swept off by the manipulator in a V-Rep environment, as shown in the Fig.~\ref{fig:V-REPenv}. Demonstrations are generated using a PID controller \cite{sellers2001pid}, similarly to the push-and-place task. A successful demonstration is defined as the manipulator sweeping away all blocks. The data collection and optimization procedure is similar to the push-and-place task, whereby after a successful demonstration, the policy and noise parameters are optimized until \ref{MGP:objective_function} converges. This procedure is repeated for 10 iterations, continuously updating the policy and noise estimates.

%Similarly to the push-and-place task, the algorithmic supervisor is a velocity controller of the robot arm using a classical PID controller as well as a push and place task \cite{sellers2001pid}.

%A demonstration describe the trajectory of a robot controlled by an algorithmic supervisor, which sweeps all the boxes out of the table in order.

%as well as the learning of probabilistic policy and the reduction of covariate shift by applying MGP-DART  sweeping three boxes on a table in a V-Rep environment as shown in the Fig.~\ref{fig:V-REPenv}.

%The goal of this task is for the robot arm to sweep the boxes out of the table to create a work-space on the table.

%After placing the boxes on the table in an arbitrary array and collecting three demonstration data sets that sweep in random order, 

%From the collection of the three demonstrations to the optimization of the policy and noise parameters in one iteration, we performed 10 iterations.
%The maximum number of iterations was determined based on the convergence of the noise parameters.

% Task setup
The task's state is the relative coordinate between the robot arm and three boxes (in 6 dimensions). An action is defined as the velocity of the robot arm in the x and y axis.

To validate the performance of MGP-DART in reducing covariate shift, 
the initial positions of three boxes were randomly placed on the table to induce scenarios in which the covariate shift tended to be large during the test episodes.
The learning models' performance was calculated as a reward for the total number of boxes out of the table at the end of the test episode (Min : 0, Max : 3).

\subsection{UR3 Manipulator}
\begin{figure}
    \centering
    % \includegraphics[width =0.7\hsize]{Figure/Realrobot/env.pdf}
    \includegraphics[width =0.7\hsize]{Figure/Realrobot/env2.pdf}
    \vspace{-2mm}
    \caption{Experimental environment for Real robot(UR3) table-sweep task. The state is the position of objects placed on the table and the action is the velocity at which the robot arm is moved.}
    \label{fig:Realenv}
\end{figure}
A final experiment, MGP-DART with the human supervisor was utilized to verify the UR3 robot can learn the task to create a workspace by sweeping office supplies (i.e. rubber tape, etc.) placed on the table as shown in Fig.~\ref{fig:Realenv}. 

The goal of this task is a robot arm sweeps the office supplies out of the table. A demonstration is a trajectory in which a robot controlled by a human expert sweeps all the office supplies out of the table in order.

Before each demonstration begins, the two objects are arbitrarily placed in a circle on the table, and the human expert controlling the robotic arm collects two demonstrations in which each office supply is swept off the table in random order and then optimizes the measure and the noise parameter until (18) is converged.
The process from collecting two demonstration datasets to the optimization of policy and noise parameters was repeated five times.

For the experiment's state, the x,y position was obtained by recognizing AR markers attached to each object (robot arm and rubber tape) through a camera. The x,y velocity of the UR3 robot arm was placed in the action.

To validate the performance of MGP-DART in reducing covariate shift, 
the initial positions of office supplies were arbitrarily placed in a circle on the table to induce scenarios in which the covariate shift tended to be large during the test episodes.
The learning models' performance was calculated as a reward for the total number of boxes out of the table at the end of the test episode (Min : 0, Max: 2).
%\clearpage

==> sections/introduction_v1.tex <==
Robot manipulation tasks in which the high-dimensional,nonlinear observations and complex dynamics models make it difficult to learn. Robot manipulation tasks is difficult to learn due to the high-dimensional, nonlinear observations and complex dynamics. Therefore, Several learning methods have been proposed for learn robot manipulation tasks to imitate human knowledge called imitation learning.

Behavioral cloning (BC) is one of the imitation learning methods in which a robot learns a control policy that imitates the human's actions by using empirical data of the human's demonstration, and it has been applied to the field of robotics \cite{bain1995framework}.
%Imitation Learning Success example
Bojarski successfully learns policy for self-driving control of cars by BC \cite{bojarski2016end}.
Zhang has also applied VR technology to BC to leverage the intuitive teleoperation and learning of complex tasks with the humanoid robot \cite{zhang2018deep}.
%Behavior Cloning Problem
%- Error compounding
%- covariate shift
However, the policy learned by BC has a distribution mismatch known as covariate shift where environmental error cause a discrepancy between the robot's training and testing phases (e.g., disturbance, model approximation error, or initial position difference). if this discrepancy grows, not only is a failure at the task, but it is also dangerous because the robot may choose actions that are damaging itself or the environment.

%=================DART=================%
Laskey et al. proposed a novel BC called Disturbances for Augmenting Robot Trajectories (DART), which injects optimized noise into the supervisor's actions when the supervisor provides a demonstration \cite{laskey2017dart}.
DART can learn a robust policy by injecting noise into the supervisor's action and encouraging the supervisor to recover from the noise.
%limitation of DART
However, DART assumes a deterministic policy model that outputs only a single action from observation to control, which is effective in elaborate tasks, but in real-world scenarios where humans stochastically choose more than one optimal action, multiple optimal actions will be averaged out \cite{bishop2006pattern}, leading to undesirable policy learning.
In DART, which leverages the approximation error of the policy model as a level of injecting noise, such policy models sometimes induce large approximation errors, which can lead to a vicious cycle of injecting unnecessarily high levels of noise into the humans in the loop.

%=================Solution=================%
As an alternative to the current DART deterministic policy model, which selects a single optimal action, a Bayesian learning framework that probabilistically infers the policy model from the data can be used to alleviate these limitations.
In a Bayesian learning framework, a policy is defined as a probability distribution of action outputs, and a probabilistic generative model of the data is constructed to probabilistically infer the posterior distribution of the policy from the supervised data based on Bayesian theory.
Gaussian Process Regression (GPR), one of the uses of Bayesian learning frameworks, deals with implicit (high-dimensional) feature spaces with kernel functions, and thus can directly deal with high-dimensional observations without having to design the feature space by hand \cite{rasmussen2003gaussian}.
In particular, Overlapping Mixtures of Gaussian Processes (OMGP) \cite{lazaro2012overlapping}, which can learn a multi-modal distribution by overlapping multiple GPs, has been employed as a policy model with multiple optimal actions in robotic policy learning, and has been applied to various tasks flexibly \cite{sasaki2019multimodal}.
Furthermore, Ross et al. proposed Infinite Overlapping Mixtures of Gaussian Processes (IOMGP) only requires an upper bound of the number of GPs to be estimated, which is more flexible than OMGP, which requires the appropriate number of mixtures to be specified in advance \cite{ross2013nonparametric}.

%=================MGP-DART=================%
Therefore, our goal is to develop a robust and flexible imitation learning framework that assumes a stochastic policy model.
We propose a Multi-modal Gaussian Process DART (MGP-DART) using a Bayesian learning framework.
We build a generative model that assumes IOMGP as the prior distribution of policies and use variational learning to train injected noise for robustness and stochastic policies in the same framework to avoid the vicious cycle of DART described above.
To verify the effectiveness of the proposed method, we have applied it in two tasks: 1) push and place task 2) table-sweep task using an algorithmic supervisor with probabilistic actions, and also applied it to the UR3 robot to learn the table-sweep task in a real environment using the human supervisor.

==> sections/introduction_v2.tex <==
Imitation learning provides a intuitive means for programming robots to perform high-level complex tasks, by enabling robots to learn skills via observation of a human expert. 
Due to the complexity of these tasks, often involving high-dimensional non-linear observations and dynamics, \textit{non-parametric mixture policies} are an attractive means to modelling policies, without prior information on the task structure. 
In addition, the use of Bayesian learning frameworks, such as Infinite Overlapping Mixtures of Gaussian Processes (IOMGP) \cite{ross2013nonparametric}, means that probabilistically inferred  policy models from the data can be used to model real-world scenarios involving stochasticity (such as multiple optimal actions). %whereby humans stochastically choose more than one optimal action.

However, the major limitation in non-parametric mixture policies, are policy errors induced by a distribution mismatch between the the robot's training and testing phases, known as \textit{covariate shift}. In this, environmental errors, such as initial position difference or state measurement error, cause a discrepancy between the learnt policy and the robot application which can result in task failure, and the generation of unsafe actions.

To address this, an intuitive approach to robustifying learnt policies against sources of error, is to exploit the phenomenon of persistence excitation \cite{} by injecting Gaussian noise into the human demonstrated actions and learning how the expert recovers from this perturbation. For tasks involving learning a deterministic policy model with single optimal actions, Disturbances for Augmenting Robot Trajectories (DART) \cite{laskey2017dart} is well suited to this, by concurrently determining the optimal noise level to be injected into the demonstrated actions during policy learning. However, this uni-model deterministic policy assumption is unsuitable for many real-world manipulation learning tasks, which may consist of multiple optimal actions. Naive application of DART to this setting can result in multiple optimal actions being averaged out \cite{bishop2006pattern}, leading to undesirable policy learning.


%In DART, which leverages the approximation error of the policy model as a level of injecting noise, such policy models sometimes induce large approximation errors, which can lead to a vicious cycle of injecting unnecessarily high levels of noise into the humans in the loop.

%=================Solution=================%
%As an alternative to the current DART deterministic policy model, which selects a single optimal action, a 

%=================MGP-DART=================%
This paper presents a robust and flexible Bayesian imitation learning framework that assumes a stochastic policy model capable of handing multiple optimal actions, referred to as Multi-modal Gaussian Process DART (MGP-DART). For this, a generative model is built, assuming an infinite overlapping mixtures of Gaussian processes as the prior distribution of policies, and variational learning is used to train injected noise for robustness and stochastic policies in the same framework. % to avoid the vicious cycle of DART described above.

To verify the effectiveness of the proposed method, experiments are presented in this paper applying the proposed method to two imitation learning tasks using a UR3 7DOF robotic arm: 1) push and place task 2) table-sweep task using an algorithmic supervisor with probabilistic actions. Experimental results show that [...], with an improvement of [...] over the state of the art method.
%. and also applied it to the UR3 robot to learn the table-sweep task in a real environment using the human supervisor.



% Method stuff

%In a Bayesian learning framework, a policy is defined as a probability distribution of action outputs, and a probabilistic generative model of the data is constructed to probabilistically infer the posterior distribution of the policy from the supervised data based on Bayesian theory.
%Gaussian Process Regression (GPR), one of the uses of Bayesian learning frameworks, deals with implicit (high-dimensional) feature spaces with kernel functions, and thus can directly deal with high-dimensional observations without having to design the feature space by hand \cite{rasmussen2003gaussian}.
%In particular, Overlapping Mixtures of Gaussian Processes (OMGP) \cite{lazaro2012overlapping}, which can learn a multi-modal distribution by overlapping multiple GPs, has been employed as a policy model with multiple optimal actions in robotic policy learning, and has been applied to various tasks flexibly \cite{sasaki2019multimodal}.
%Furthermore, Ross et al. proposed Infinite Overlapping Mixtures of Gaussian Processes (IOMGP) only requires an upper bound of the number of GPs to be estimated, which is more flexible than OMGP, which requires the appropriate number of mixtures to be specified in advance \cite{ross2013nonparametric}.




%Robot manipulation tasks in which the high-dimensional,nonlinear observations and complex dynamics models make it difficult to learn. Robot manipulation tasks is difficult to learn due to the high-dimensional, nonlinear observations and complex dynamics. Therefore, Several learning methods have been proposed for learn robot manipulation tasks to imitate human knowledge called imitation learning.


%Behavioral cloning (BC) is one of the imitation learning methods in which a robot learns a control policy that imitates the human's actions by using empirical data of the human's demonstration, and it has been applied to the field of robotics \cite{bain1995framework}.

%Imitation Learning Success example
%Bojarski successfully learns policy for self-driving control of cars by BC \cite{bojarski2016end}.
%Zhang has also applied VR technology to BC to leverage the intuitive teleoperation and learning of complex tasks with the humanoid robot \cite{zhang2018deep}.



%Behavior Cloning Problem
%- Error compounding
%- covariate shift


==> sections/introduction_v3.tex <==
% Introduction of IL
Imitation learning provides an attractive means for programming robots to perform complex high-level tasks, by enabling robots to learn skills via observation of an expert demonstrator \cite{coates2009apprenticeship,bojarski2016end,zhang2018deep,osa2018algorithmic}.
%Through learning by demonstration, imitation learning has been successfully applied in many complex applications in which it would be difficult to create analytical control strategies, including  helicopter controllers \cite{coates2009apprenticeship}, self-driving cars  \cite{bojarski2016end}, and humanoid robots \cite{zhang2018deep}.
% \textit{Behavioral cloning} (BC) is one of an imitation learning approach in which a method for directly regressing a policy from training data collected by a human expert \cite{bain1995framework}.
However, two significant limitations of this approach severely limit applicability to real-world scenarios, these being: 
\begin{inparaenum}
\item learning policies from a human expert demonstrator is often very complex, as humans often choose between multiple optimal actions, and
\item even with an optimally learnt control model, policies can be vulnerable to compounding errors during online operation (\ie there is a lack of robustness).
\end{inparaenum}
In the former, uncertainties and stochastic behaviour of the human expert (e.g. multiple optimal actions for a given task), increase the complexity of learning policies, and as such, \textit{flexible policy models} are needed to capture such complexity. In the latter case, compounding errors from environmental variations (e.g. task starting position), may induce significant difference between the expert's training distribution, and the applied policy. This drifting issue is commonly referred to as covariate shift \cite{ross2010efficient}, and requires \textit{robust policy models}.

To address both these limitations, this paper presents a novel Bayesian imitation learning framework,  that learns a stochastic policy model capable of being both flexible to variations in expert demonstrations, and robust to sources of error in policy application. This is referred to as Multi-modal Gaussian Process DART (MGP-DART).

Specifically, complex human policies (often involving high-dimensional non-linear observations and dynamics) are modelled using \textit{probablistic non-parametric mixture policies} \cite{ross2013nonparametric}. To robustify the learnt policies against sources of error, the phenomenon of persistence excitation \cite{sastry2011adaptive} is exploited, by injecting noise into the human demonstrated actions and learning how the expert recovers from this perturbation. Given this conceptual framework, a \textit{pseudo-generative model} of the estimated noiseless expert action is derived, and in the same schema, variational learning is used to train the injected noise for robustness and stochastic policies.

% via a maximum likelihood is built assuming an IOMGP as the prior distribution of policies


%For tasks involving learning a deterministic policy model with single optimal actions, Disturbances for Augmenting Robot Trajectories (DART) \cite{laskey2017dart} is well suited to this concurrently determining the optimal noise level to be injected into the demonstrated actions during policy learning.







%address both the complexity of the human-policies and the vulnerability of the learned-policies, based on a Bayesian learning framework. 


%In DART, which leverages the approximation error of the policy model as a level of injecting noise, such policy models sometimes induce large approximation errors, which can lead to a vicious cycle of injecting unnecessarily high levels of noise into the humans in the loop.

%=================Solution=================%
%As an alternative to the current DART deterministic policy model, which selects a single optimal action, a 

%=================MGP-DART=================%


To evaluate the effectiveness of the proposed method, experiments are carried out on two imitation learning tasks using a UR3 7DOF robotic arm, these being a: 
\begin{inparaenum}
\item push and place task, 
\item table-sweep task using an algorithmic supervisor with probabilistic action.
\end{inparaenum}
Results show that, through improved flexibility and robustness, the learning performance and control safety are better than comparison methods (i.e., methods that do not consider flexibility and robustness simultaneously).


% Method stuff

%In a Bayesian learning framework, a policy is defined as a probability distribution of action outputs, and a probabilistic generative model of the data is constructed to probabilistically infer the posterior distribution of the policy from the supervised data based on Bayesian theory.
%Gaussian Process Regression (GPR), one of the uses of Bayesian learning frameworks, deals with implicit (high-dimensional) feature spaces with kernel functions, and thus can directly deal with high-dimensional observations without having to design the feature space by hand \cite{rasmussen2003gaussian}.
%In particular, Overlapping Mixtures of Gaussian Processes (OMGP) \cite{lazaro2012overlapping}, which can learn a multi-modal distribution by overlapping multiple GPs, has been employed as a policy model with multiple optimal actions in robotic policy learning, and has been applied to various tasks flexibly \cite{sasaki2019multimodal}.
%Furthermore, Ross et al. proposed Infinite Overlapping Mixtures of Gaussian Processes (IOMGP) only requires an upper bound of the number of GPs to be estimated, which is more flexible than OMGP, which requires the appropriate number of mixtures to be specified in advance \cite{ross2013nonparametric}.




%Robot manipulation tasks in which the high-dimensional,nonlinear observations and complex dynamics models make it difficult to learn. Robot manipulation tasks is difficult to learn due to the high-dimensional, nonlinear observations and complex dynamics. Therefore, Several learning methods have been proposed for learn robot manipulation tasks to imitate human knowledge called imitation learning.


%Behavioral cloning (BC) is one of the imitation learning methods in which a robot learns a control policy that imitates the human's actions by using empirical data of the human's demonstration, and it has been applied to the field of robotics \cite{bain1995framework}.

%Imitation Learning Success example
%Bojarski successfully learns policy for self-driving control of cars by BC \cite{bojarski2016end}.
%Zhang has also applied VR technology to BC to leverage the intuitive teleoperation and learning of complex tasks with the humanoid robot \cite{zhang2018deep}.



%Behavior Cloning Problem
%- Error compounding
%- covariate shift

